Scalable Nonlinear Learning with Adaptive Polynomial Expansions

Can we effectively learn a nonlinear representation in time comparable to linear learning? We describe a new algorithm that explicitly and adaptively expands higher-order interaction features over base linear representations. The algorithm is designed for extreme computational efficiency, and an extensive experimental study shows that its computation/prediction tradeoff ability compares very favorably against strong baselines.

==> __includes.tex <==
\usepackage{amsmath,amsbsy,amsfonts,amssymb,amsthm,color,dsfont}
%\usepackage{fullpage}

\newcommand\lectureheader[5]{{\noindent\framebox[\textwidth]{%
\begin{minipage}{0.98\textwidth}%
\textsf{#1 \hfill #2}%
\vspace{-0.5cm}%
\begin{center}%
\Large\textsf{\textbf{#3}}%
\end{center}%
\vspace{-0.2cm}%
\textsf{\emph{#4 \hfill #5}}%
\end{minipage}%
}\bigskip}}

\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}

% \bA, \bB, ...
\def\ddef#1{\expandafter\def\csname b#1\endcsname{\ensuremath{\mathbf{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

% \bbA, \bbB, ...
\def\ddef#1{\expandafter\def\csname bb#1\endcsname{\ensuremath{\mathbb{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

% \cA, \cB, ...
\def\ddef#1{\expandafter\def\csname c#1\endcsname{\ensuremath{\mathcal{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

% \vA, \vB, ..., \va, \vb, ...
\def\ddef#1{\expandafter\def\csname v#1\endcsname{\ensuremath{\boldsymbol{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz\ddefloop

% \valpha, \vbeta, ...,  \vGamma, \vDelta, ...,
\def\ddef#1{\expandafter\def\csname v#1\endcsname{\ensuremath{\boldsymbol{\csname #1\endcsname}}}}
\ddefloop {alpha}{beta}{gamma}{delta}{epsilon}{varepsilon}{zeta}{eta}{theta}{vartheta}{iota}{kappa}{lambda}{mu}{nu}{xi}{pi}{varpi}{rho}{varrho}{sigma}{varsigma}{tau}{upsilon}{phi}{varphi}{chi}{psi}{omega}{Gamma}{Delta}{Theta}{Lambda}{Xi}{Pi}{Sigma}{varSigma}{Upsilon}{Phi}{Psi}{Omega}\ddefloop

\newcommand\B{\ensuremath{\mathbb{B}}}
\newcommand\E{\ensuremath{\mathbb{E}}}
\newcommand\N{\ensuremath{\mathbb{N}}}
\renewcommand\P{\ensuremath{\mathbb{P}}}
\newcommand\R{\ensuremath{\mathbb{R}}}
\newcommand\C{\ensuremath{\mathbb{C}}}
\renewcommand\S{\ensuremath{\mathbb{S}}}

\newcommand\Normal{\ensuremath{\mathcal{N}}}
\newcommand\Bernoulli{\ensuremath{\operatorname{Bernoulli}}}

\newcommand\Sig{\ensuremath{\varSigma}}
\newcommand\veps{\ensuremath{\varepsilon}}
\newcommand\eps{\ensuremath{\epsilon}}

\renewcommand\t{{\ensuremath{\scriptscriptstyle{\top}}}}
\newcommand\ind[1]{\ensuremath{\mathds{1}\{#1\}}}
\newcommand\dotp[1]{\langle #1 \rangle}

\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Diag}{Diag}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\vol}{vol}

\DeclareMathOperator{\var}{var}

\DeclareMathOperator{\Bd}{bd}
\DeclareMathOperator{\Cl}{cl}
\DeclareMathOperator{\Conv}{conv}
\DeclareMathOperator{\Int}{int}
\DeclareMathOperator{\Null}{ker}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\Range}{ran}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand\wt{\ensuremath{\widetilde}}
\newcommand\wh{\ensuremath{\widehat}}
\renewcommand\v{\ensuremath{\boldsymbol}}

\newcommand\comment[1]{{\color{blue}\{\emph{Comment}:} #1{\color{blue}\}}}

\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\theoremstyle{remark}
\newtheorem{remark}{Remark}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{condition}{Condition}
\newtheorem{example}{Example}
\newtheorem{problem}{Problem}

\newcommand\parens[1]{\left( #1 \right)}
\newcommand\norm[1]{\left\| #1 \right\|}
\newcommand\braces[1]{\left\{ #1 \right\}}
\newcommand\brackets[1]{\left[ #1 \right]}
\newcommand\ceil[1]{\left\lceil #1 \right\rceil}



==> summary_small_2.tex <==
\begin{tabular} {|c|c|c|c|c|c|c|c|c|} \hline 
~& \lalg & \qalg & \calg & \alg (1) & \alg (0.75) & \alg (0.5) & \alg (0.25) & \alg (0.125) \\ \hline 
 \multirow{2}{*}{bio} & 3.122e-03 & 3.122e-03 & 3.087e-03 & 2.985e-03 & 3.053e-03 & 2.985e-03 & 3.259e-03 & 3.156e-03  \\ 
& 2.644e+00  & 5.000e+00  & 5.965e+02  & 3.036e+00  & 3.340e+00  & 7.516e+00  & 1.841e+01  & 4.745e+01   \\ \hline
 \multirow{2}{*}{a9a} & 1.510e-01 & 1.485e-01 & 1.496e-01 & 1.488e-01 & 1.488e-01 & 1.489e-01 & 1.478e-01 & 1.481e-01  \\ 
& 3.880e-01  & 4.320e-01  & 4.176e+00  & 2.840e-01  & 3.000e-01  & 4.880e-01  & 4.040e-01  & 4.080e-01   \\ \hline
 \multirow{2}{*}{adult} & 1.557e-01 & 1.529e-01 & 1.531e-01 & 1.525e-01 & 1.525e-01 & 1.507e-01 & 1.513e-01 & 1.474e-01  \\ 
& 3.440e-01  & 4.520e-01  & 4.252e+00  & 2.480e-01  & 2.400e-01  & 3.680e-01  & 3.920e-01  & 4.040e-01   \\ \hline
 \multirow{2}{*}{titanic} & 2.182e-01 & 2.136e-01 & 2.136e-01 & 2.136e-01 & 2.136e-01 & 2.136e-01 & 2.136e-01 & 2.136e-01  \\ 
& 1.600e-02  & 2.000e-02  & 9.601e-02  & 2.800e-02  & 3.600e-02  & 4.000e-02  & 3.200e-02  & 3.600e-02   \\ \hline
 \multirow{2}{*}{kdda} & 1.240e-01 & 1.272e-01 & 1.253e-01 & 1.240e-01 & 1.240e-01 & 1.240e-01 & 1.240e-01 & 1.240e-01  \\ 
& 9.492e+01  & 3.715e+02  & 3.266e+04  & 7.629e+01  & 6.689e+01  & 8.318e+01  & 5.768e+01  & 8.463e+01   \\ \hline
 \multirow{2}{*}{census} & 4.748e-02 & 4.579e-02 & 4.651e-02 & 4.674e-02 & 4.686e-02 & 4.698e-02 & 4.586e-02 & 4.648e-02  \\ 
& 3.068e+00  & 7.784e+00  & 5.754e+02  & 2.200e+00  & 2.180e+00  & 2.144e+00  & 2.532e+00  & 3.936e+00   \\ \hline
 \multirow{2}{*}{20news} & 8.119e-02 & 8.437e-02 & 8.384e-02 & 8.437e-02 & 9.021e-02 & 1.210e-01 & 9.525e-02 & 7.986e-02  \\ 
& 5.440e-01  & 2.303e+01  & 5.262e+04  & 6.440e-01  & 6.480e-01  & 8.121e-01  & 1.040e+00  & 2.112e+00   \\ \hline
 \multirow{2}{*}{abalone\_bin} & 2.898e-01 & 2.826e-01 & 2.719e-01 & 2.874e-01 & 2.874e-01 & 2.766e-01 & 2.743e-01 & 2.754e-01  \\ 
& 4.400e-02  & 4.000e-02  & 2.440e-01  & 6.000e-02  & 4.400e-02  & 6.400e-02  & 6.800e-02  & 1.080e-01   \\ \hline
 \multirow{2}{*}{year} & 1.157e-02 & 1.073e-02 & 1.113e-02 & 1.112e-02 & 1.099e-02 & 1.083e-02 & 1.069e-02 & 1.060e-02  \\ 
& 1.261e+01  & 6.915e+01  & 1.136e+04  & 1.529e+01  & 2.201e+01  & 4.585e+01  & 1.189e+02  & 4.179e+02   \\ \hline
 \multirow{2}{*}{poker} & 4.555e-01 & 4.091e-01 & 4.100e-01 & 4.119e-01 & 4.119e-01 & 4.092e-01 & 4.099e-01 & 4.085e-01  \\ 
& 4.388e+00  & 6.736e+00  & 2.294e+01  & 6.228e+00  & 3.836e+00  & 6.516e+00  & 1.230e+01  & 1.657e+01   \\ \hline
 \multirow{2}{*}{abalone\_reg} & 8.052e+00 & 7.489e+00 & 7.107e+00 & 7.812e+00 & 7.812e+00 & 7.690e+00 & 7.003e+00 & 6.740e+00  \\ 
& 4.000e-02  & 4.400e-02  & 1.680e-01  & 5.600e-02  & 5.600e-02  & 5.600e-02  & 7.200e-02  & 8.400e-02   \\ \hline
 \multirow{2}{*}{kddcup2009} & 7.310e-02 & 7.310e-02 & 7.310e-02 & 7.310e-02 & 7.310e-02 & 7.310e-02 & 7.310e-02 & 7.310e-02  \\ 
& 7.600e-01  & 1.144e+01  & 1.213e+03  & 9.801e-01  & 1.196e+00  & 1.208e+00  & 1.204e+00  & 8.881e-01   \\ \hline
 \multirow{2}{*}{covtype} & 2.450e-01 & 2.184e-01 & 2.039e-01 & 2.331e-01 & 2.331e-01 & 2.287e-01 & 2.261e-01 & 2.208e-01  \\ 
& 4.444e+00  & 3.116e+00  & 2.133e+01  & 4.204e+00  & 4.488e+00  & 2.856e+00  & 5.120e+00  & 4.192e+00   \\ \hline
 \multirow{2}{*}{w8a} & 1.538e-02 & 1.246e-02 & 1.337e-02 & 1.518e-02 & 1.518e-02 & 1.417e-02 & 1.317e-02 & 1.286e-02  \\ 
& 1.320e-01  & 4.520e-01  & 1.448e+01  & 2.760e-01  & 3.520e-01  & 3.120e-01  & 1.480e-01  & 1.960e-01   \\ \hline
 \multirow{2}{*}{nomao} & 6.325e-02 & 5.063e-02 & 5.107e-02 & 5.992e-02 & 5.701e-02 & 5.513e-02 & 4.933e-02 & 4.904e-02  \\ 
& 5.000e-01  & 3.564e+00  & 7.038e+02  & 6.120e-01  & 7.480e-01  & 1.280e+00  & 2.900e+00  & 6.348e+00   \\ \hline
 \multirow{2}{*}{magic04} & 2.142e-01 & 1.672e-01 & 1.638e-01 & 1.880e-01 & 1.880e-01 & 1.801e-01 & 1.706e-01 & 1.696e-01  \\ 
& 1.040e-01  & 1.400e-01  & 5.480e-01  & 1.960e-01  & 1.760e-01  & 1.520e-01  & 2.600e-01  & 3.560e-01   \\ \hline
 \multirow{2}{*}{rcv1} & 4.860e-02 & 4.060e-02 & 3.701e-02 & 4.570e-02 & 4.511e-02 & 4.438e-02 & 4.273e-02 & 4.205e-02  \\ 
& 1.627e+01  & 1.823e+02  & 6.251e+04  & 1.895e+01  & 1.977e+01  & 2.171e+01  & 2.401e+01  & 3.671e+01   \\ \hline
 \multirow{2}{*}{letter} & 2.273e-01 & 1.918e-01 & 1.688e-01 & 1.872e-01 & 1.878e-01 & 1.727e-01 & 1.670e-01 & 1.638e-01  \\ 
& 1.440e-01  & 2.040e-01  & 1.376e+00  & 1.680e-01  & 1.920e-01  & 3.000e-01  & 4.280e-01  & 6.800e-01   \\ \hline
 \multirow{2}{*}{vehv2binary} & 3.400e-02 & 2.670e-02 & 2.505e-02 & 8.337e-03 & 8.087e-03 & 8.772e-03 & 1.109e-02 & 1.151e-02  \\ 
& 3.364e+00  & 9.065e+00  & 1.079e+03  & 2.880e+00  & 4.076e+00  & 8.105e+00  & 1.825e+01  & 4.065e+01   \\ \hline
 \multirow{2}{*}{comp} & 3.409e-03 & 2.627e-03 & 3.662e-03 & 2.587e-03 & 2.587e-03 & 2.124e-03 & 2.038e-03 & 2.070e-03  \\ 
& 7.601e-02  & 8.000e-02  & 3.560e-01  & 6.401e-02  & 6.400e-02  & 1.240e-01  & 1.080e-01  & 1.560e-01   \\ \hline
 \multirow{2}{*}{cal\_housing} & 7.410e-02 & 8.651e-02 & 1.055e-01 & 9.414e-02 & 9.414e-02 & 9.856e-02 & 9.881e-02 & 1.183e-01  \\ 
& 9.201e-02  & 1.680e-01  & 4.000e-01  & 1.080e-01  & 1.080e-01  & 2.120e-01  & 2.600e-01  & 3.360e-01   \\ \hline
 \multirow{2}{*}{cup98} & 5.697e-02 & 3.841e-02 & 4.215e-02 & 5.646e-02 & 5.687e-02 & 6.450e-02 & 6.780e-02 & 5.948e-02  \\ 
& 3.452e+00  & 1.342e+02  & 1.010e+05  & 4.736e+00  & 4.180e+00  & 4.240e+00  & 4.504e+00  & 7.084e+00   \\ \hline
 \multirow{2}{*}{maptaskcoref} & 1.087e-01 & 7.553e-02 & 6.598e-02 & 9.997e-02 & 9.805e-02 & 9.691e-02 & 9.338e-02 & 8.083e-02  \\ 
& 9.361e-01  & 6.412e+00  & 7.504e+02  & 1.424e+00  & 1.424e+00  & 1.856e+00  & 2.628e+00  & 3.240e+00   \\ \hline
 \multirow{2}{*}{eeg\_eye\_state} & 3.815e-01 & 2.573e-01 & 2.300e-01 & 3.127e-01 & 3.127e-01 & 2.557e-01 & 2.383e-01 & 2.136e-01  \\ 
& 1.360e-01  & 2.000e-01  & 7.960e-01  & 1.840e-01  & 1.640e-01  & 2.040e-01  & 2.920e-01  & 5.160e-01   \\ \hline
 \multirow{2}{*}{activity} & 1.298e-02 & 8.422e-03 & 6.762e-03 & 8.694e-03 & 5.856e-03 & 5.977e-03 & 4.951e-03 & 4.166e-03  \\ 
& 5.560e-01  & 9.921e-01  & 7.864e+00  & 1.116e+00  & 1.048e+00  & 1.828e+00  & 2.304e+00  & 4.564e+00   \\ \hline
 \multirow{2}{*}{ijcnn1} & 7.942e-02 & 4.501e-02 & 3.481e-02 & 5.221e-02 & 5.221e-02 & 4.041e-02 & 3.921e-02 & 3.901e-02  \\ 
& 2.000e-01  & 1.800e-01  & 6.960e-01  & 2.200e-01  & 1.800e-01  & 1.840e-01  & 3.080e-01  & 3.000e-01   \\ \hline
 \multirow{2}{*}{shuttle} & 2.644e-02 & 1.391e-02 & 9.195e-03 & 1.218e-02 & 1.218e-02 & 5.402e-03 & 1.023e-02 & 7.931e-03  \\ 
& 1.040e-01  & 1.240e-01  & 4.160e-01  & 2.680e-01  & 2.520e-01  & 3.000e-01  & 3.360e-01  & 3.080e-01   \\ \hline
 \multirow{2}{*}{slice} & 7.243e-03 & 1.403e-03 & 7.797e-04 & 5.095e-03 & 3.455e-03 & 2.302e-03 & 1.825e-03 & 1.196e-03  \\ 
& 1.600e+00  & 3.303e+01  & 7.944e+03  & 1.972e+00  & 2.168e+00  & 4.880e+00  & 1.609e+01  & 3.709e+01   \\ \hline
 \multirow{2}{*}{skin} & 7.421e-02 & 1.045e-02 & 5.835e-03 & 2.165e-02 & 2.165e-02 & 2.165e-02 & 1.585e-02 & 7.366e-03  \\ 
& 4.600e-01  & 1.148e+00  & 1.220e+00  & 5.400e-01  & 1.220e+00  & 1.276e+00  & 6.280e-01  & 1.384e+00   \\ \hline
 \multirow{2}{*}{mushroom} & 5.723e-02 & 5.538e-03 & 6.154e-04 & 6.646e-02 & 9.108e-02 & 4.923e-02 & 1.538e-02 & 1.846e-02  \\ 
& 7.200e-02  & 6.800e-02  & 2.788e+00  & 8.001e-02  & 5.600e-02  & 6.000e-02  & 1.320e-01  & 1.760e-01   \\ \hline
\end{tabular}

==> summary_table1.tex <==
\begin{tabular} {|c|c|c|c|c|c|c|c|c|} \hline 
~& \lalg & \qalg & \calg & \alg (1) & \alg (0.75) & \alg (0.5) & \alg (0.25) & \alg (0.125) \\ \hline 
 \multirow{2}{*}{bio} & 3.122e-03 & 3.122e-03 & 3.087e-03 & 2.985e-03 & 3.053e-03 & 2.985e-03 & 3.259e-03 & 3.087e-03  \\ 
& 2.672e+00  & 5.396e+00  & 4.068e+02  & 3.800e+00  & 4.040e+00  & 8.141e+00  & 1.903e+01  & 4.963e+01   \\ \hline
 \multirow{2}{*}{a9a} & 1.510e-01 & 1.485e-01 & 1.496e-01 & 1.488e-01 & 1.488e-01 & 1.489e-01 & 1.478e-01 & 1.481e-01  \\ 
& 4.120e-01  & 4.880e-01  & 3.508e+00  & 4.720e-01  & 4.440e-01  & 3.840e-01  & 4.640e-01  & 3.560e-01   \\ \hline
 \multirow{2}{*}{adult} & 1.557e-01 & 1.529e-01 & 1.531e-01 & 1.525e-01 & 1.525e-01 & 1.507e-01 & 1.513e-01 & 1.474e-01  \\ 
& 2.240e-01  & 3.800e-01  & 4.256e+00  & 3.000e-01  & 2.680e-01  & 2.840e-01  & 4.680e-01  & 4.520e-01   \\ \hline
 \multirow{2}{*}{titanic} & 2.182e-01 & 2.136e-01 & 2.136e-01 & 2.136e-01 & 2.136e-01 & 2.136e-01 & 2.136e-01 & 2.136e-01  \\ 
& 2.000e-02  & 1.600e-02  & 1.040e-01  & 2.400e-02  & 2.400e-02  & 3.200e-02  & 3.200e-02  & 2.800e-02   \\ \hline
 \multirow{2}{*}{kdda} & 1.240e-01 & 1.272e-01 & 1.253e-01 & 1.240e-01 & 1.240e-01 & 1.240e-01 & 1.240e-01 & 1.240e-01  \\ 
& 7.164e+01  & 2.676e+02  & 3.231e+04  & 7.397e+01  & 6.044e+01  & 6.148e+01  & 6.128e+01  & 8.257e+01   \\ \hline
 \multirow{2}{*}{census} & 4.748e-02 & 4.579e-02 & 4.651e-02 & 4.674e-02 & 4.686e-02 & 4.698e-02 & 4.586e-02 & 4.648e-02  \\ 
& 2.300e+00  & 6.560e+00  & 3.848e+02  & 1.936e+00  & 3.152e+00  & 2.104e+00  & 3.136e+00  & 5.212e+00   \\ \hline
 \multirow{2}{*}{20news} & 8.119e-02 & 8.437e-02 & 8.384e-02 & 8.437e-02 & 9.021e-02 & 1.210e-01 & 9.525e-02 & 7.986e-02  \\ 
& 5.320e-01  & 1.119e+01  & 5.609e+04  & 8.081e-01  & 7.600e-01  & 8.761e-01  & 1.080e+00  & 1.656e+00   \\ \hline
 \multirow{2}{*}{abalone\_bin} & 2.898e-01 & 2.826e-01 & 2.719e-01 & 2.874e-01 & 2.874e-01 & 2.766e-01 & 2.743e-01 & 2.754e-01  \\ 
& 4.000e-02  & 4.400e-02  & 1.360e-01  & 4.000e-02  & 6.400e-02  & 5.600e-02  & 9.201e-02  & 7.601e-02   \\ \hline
 \multirow{2}{*}{year} & 1.157e-02 & 1.073e-02 & 1.113e-02 & 1.112e-02 & 1.099e-02 & 1.083e-02 & 1.069e-02 & 1.060e-02  \\ 
& 1.164e+01  & 7.316e+01  & 1.443e+04  & 1.830e+01  & 2.688e+01  & 4.885e+01  & 1.318e+02  & 2.659e+02   \\ \hline
 \multirow{2}{*}{poker} & 4.555e-01 & 4.091e-01 & 4.100e-01 & 4.119e-01 & 4.119e-01 & 4.093e-01 & 4.099e-01 & 4.085e-01  \\ 
& 2.536e+00  & 4.404e+00  & 1.979e+01  & 7.240e+00  & 4.180e+00  & 7.464e+00  & 1.212e+01  & 1.636e+01   \\ \hline
 \multirow{2}{*}{abalone\_reg} & 8.052e+00 & 7.489e+00 & 7.107e+00 & 7.812e+00 & 7.812e+00 & 7.690e+00 & 7.003e+00 & 6.740e+00  \\ 
& 3.200e-02  & 2.400e-02  & 1.360e-01  & 4.800e-02  & 4.000e-02  & 5.200e-02  & 5.600e-02  & 9.201e-02   \\ \hline
 \multirow{2}{*}{kddcup2009} & 7.310e-02 & 8.420e-02 & 7.310e-02 & 7.310e-02 & 7.310e-02 & 7.310e-02 & 7.310e-02 & 7.310e-02  \\ 
& 5.520e-01  & 4.368e+00  & 7.459e+02  & 1.096e+00  & 1.380e+00  & 2.092e+00  & 4.356e+00  & 5.316e+00   \\ \hline
 \multirow{2}{*}{covtype} & 2.450e-01 & 2.184e-01 & 2.039e-01 & 2.331e-01 & 2.331e-01 & 2.287e-01 & 2.261e-01 & 2.208e-01  \\ 
& 3.748e+00  & 3.236e+00  & 1.961e+01  & 4.316e+00  & 4.052e+00  & 5.236e+00  & 4.212e+00  & 7.048e+00   \\ \hline
 \multirow{2}{*}{w8a} & 1.538e-02 & 1.246e-02 & 1.337e-02 & 1.518e-02 & 1.518e-02 & 1.417e-02 & 1.317e-02 & 1.286e-02  \\ 
& 1.200e-01  & 2.760e-01  & 1.185e+01  & 2.960e-01  & 1.880e-01  & 1.800e-01  & 2.120e-01  & 1.760e-01   \\ \hline
 \multirow{2}{*}{nomao} & 6.325e-02 & 5.063e-02 & 5.107e-02 & 5.992e-02 & 5.701e-02 & 5.513e-02 & 4.933e-02 & 4.904e-02  \\ 
& 5.520e-01  & 2.964e+00  & 4.944e+02  & 7.120e-01  & 1.004e+00  & 1.608e+00  & 3.108e+00  & 4.880e+00   \\ \hline
\end{tabular}


==> summary_table2.tex <==
\begin{tabular} {|c|c|c|c|c|c|c|c|c|} \hline 
~& \lalg & \qalg & \calg & \alg (1) & \alg (0.75) & \alg (0.5) & \alg (0.25) & \alg (0.125) \\ \hline 
 \multirow{2}{*}{magic04} & 2.142e-01 & 1.672e-01 & 1.638e-01 & 1.880e-01 & 1.880e-01 & 1.801e-01 & 1.706e-01 & 1.696e-01  \\ 
& 1.640e-01  & 1.200e-01  & 4.920e-01  & 1.640e-01  & 1.200e-01  & 2.800e-01  & 3.240e-01  & 3.600e-01   \\ \hline
 \multirow{2}{*}{rcv1} & 4.860e-02 & 4.061e-02 & 3.701e-02 & 4.570e-02 & 4.511e-02 & 4.438e-02 & 4.273e-02 & 4.205e-02  \\ 
& 1.906e+01  & 1.029e+02  & 6.658e+04  & 1.765e+01  & 1.790e+01  & 2.148e+01  & 2.506e+01  & 3.511e+01   \\ \hline
 \multirow{2}{*}{letter} & 2.273e-01 & 1.918e-01 & 1.688e-01 & 1.872e-01 & 1.878e-01 & 1.727e-01 & 1.670e-01 & 1.638e-01  \\ 
& 8.401e-02  & 1.560e-01  & 1.192e+00  & 1.800e-01  & 2.800e-01  & 2.760e-01  & 3.560e-01  & 5.880e-01   \\ \hline
 \multirow{2}{*}{vehv2binary} & 3.400e-02 & 2.670e-02 & 2.505e-02 & 8.337e-03 & 8.087e-03 & 8.772e-03 & 1.109e-02 & 1.151e-02  \\ 
& 2.668e+00  & 8.553e+00  & 5.269e+02  & 4.480e+00  & 3.520e+00  & 1.016e+01  & 1.709e+01  & 4.583e+01   \\ \hline
 \multirow{2}{*}{comp} & 3.409e-03 & 2.627e-03 & 3.663e-03 & 2.587e-03 & 2.587e-03 & 2.124e-03 & 2.038e-03 & 2.146e-03  \\ 
& 7.600e-02  & 7.200e-02  & 3.400e-01  & 6.401e-02  & 6.000e-02  & 1.120e-01  & 1.360e-01  & 2.200e-01   \\ \hline
 \multirow{2}{*}{cal\_housing} & 7.410e-02 & 8.651e-02 & 1.055e-01 & 9.414e-02 & 9.414e-02 & 9.856e-02 & 1.017e-01 & 1.183e-01  \\ 
& 1.120e-01  & 1.280e-01  & 5.400e-01  & 1.320e-01  & 1.560e-01  & 2.640e-01  & 2.720e-01  & 3.120e-01   \\ \hline
 \multirow{2}{*}{cup98} & 5.697e-02 & 3.841e-02 & 4.217e-02 & 5.646e-02 & 5.687e-02 & 6.450e-02 & 6.780e-02 & 5.948e-02  \\ 
& 3.448e+00  & 8.344e+01  & 1.028e+05  & 4.240e+00  & 4.692e+00  & 5.432e+00  & 5.448e+00  & 5.280e+00   \\ \hline
 \multirow{2}{*}{maptaskcoref} & 1.087e-01 & 7.553e-02 & 6.598e-02 & 9.997e-02 & 9.805e-02 & 9.691e-02 & 9.338e-02 & 8.083e-02  \\ 
& 8.801e-01  & 7.156e+00  & 4.343e+02  & 1.712e+00  & 1.164e+00  & 1.788e+00  & 2.340e+00  & 2.716e+00   \\ \hline
 \multirow{2}{*}{eeg\_eye\_state} & 3.815e-01 & 2.573e-01 & 2.300e-01 & 3.127e-01 & 3.127e-01 & 2.557e-01 & 2.383e-01 & 2.136e-01  \\ 
& 1.480e-01  & 1.640e-01  & 8.001e-01  & 1.400e-01  & 1.560e-01  & 1.800e-01  & 3.360e-01  & 4.360e-01   \\ \hline
 \multirow{2}{*}{activity} & 1.298e-02 & 8.422e-03 & 6.762e-03 & 8.694e-03 & 5.856e-03 & 5.977e-03 & 4.951e-03 & 4.166e-03  \\ 
& 9.201e-01  & 1.192e+00  & 8.313e+00  & 7.760e-01  & 1.400e+00  & 1.264e+00  & 2.928e+00  & 4.176e+00   \\ \hline
 \multirow{2}{*}{ijcnn1} & 7.942e-02 & 4.501e-02 & 3.481e-02 & 5.221e-02 & 5.221e-02 & 4.041e-02 & 3.921e-02 & 3.901e-02  \\ 
& 1.920e-01  & 2.600e-01  & 5.760e-01  & 2.440e-01  & 1.720e-01  & 2.120e-01  & 3.280e-01  & 4.080e-01   \\ \hline
 \multirow{2}{*}{shuttle} & 2.644e-02 & 1.391e-02 & 9.195e-03 & 1.218e-02 & 1.218e-02 & 5.402e-03 & 1.023e-02 & 7.931e-03  \\ 
& 2.400e-01  & 1.160e-01  & 3.080e-01  & 1.120e-01  & 1.200e-01  & 2.480e-01  & 2.960e-01  & 3.920e-01   \\ \hline
 \multirow{2}{*}{slice} & 7.243e-03 & 1.403e-03 & 7.797e-04 & 5.095e-03 & 3.455e-03 & 2.302e-03 & 1.827e-03 & 1.196e-03  \\ 
& 1.840e+00  & 2.078e+01  & 7.482e+03  & 2.132e+00  & 1.928e+00  & 6.148e+00  & 1.532e+01  & 3.095e+01   \\ \hline
 \multirow{2}{*}{skin} & 7.421e-02 & 1.045e-02 & 5.835e-03 & 2.165e-02 & 2.165e-02 & 2.165e-02 & 1.585e-02 & 7.366e-03  \\ 
& 3.800e-01  & 6.440e-01  & 4.600e-01  & 5.320e-01  & 5.720e-01  & 1.204e+00  & 7.840e-01  & 1.424e+00   \\ \hline
 \multirow{2}{*}{mushroom} & 5.354e-02 & 5.538e-03 & 6.154e-04 & 6.585e-02 & 8.862e-02 & 4.923e-02 & 2.154e-02 & 1.846e-02  \\ 
& 7.601e-02  & 9.201e-02  & 3.480e+00  & 6.800e-02  & 7.200e-02  & 6.000e-02  & 1.120e-01  & 1.920e-01   \\ \hline
\end{tabular}

